Machine Learning Interpretability Meets TLS Fingerprinting

Protecting users' privacy over the Internet is of great importance; however, it becomes harder and harder to maintain due to the increasing complexity of network protocols and components. Therefore, investigating and understanding how data is leaked from the information transmission platforms and protocols can lead us to a more secure environment. In this paper, we propose a framework to systematically find the most vulnerable information fields in a network protocol. To this end, focusing on the transport layer security (TLS) protocol, we perform different machine-learning-based fingerprinting attacks on the collected data from more than 70 domains (websites) to understand how and where this information leakage occurs in the TLS protocol. Then, by employing the interpretation techniques developed in the machine learning community and applying our framework, we find the most vulnerable information fields in the TLS protocol. Our findings demonstrate that the TLS handshake (which is mainly unencrypted), the TLS record length appearing in the TLS application data header, and the initialization vector (IV) field are among the most critical leaker parts in this protocol, respectively.

==> 03-background.tex <==
\subsection{Deep Learning}
\mahdiC{Do we need such subsection?}
In this section, we explain some preliminary subjects about Deep learning. Also We introduce Deep Neural Networks (DNN), Convolutional Neural Networks (CNN), and Recurrent Neural Networks (RNN).

Machine Learning algorithms have created breakthrough advancements in many scientific areas such as computer vision and drug discovery. After the successful applications of classical Machine Learning algorithms like support vector machines, random forest, and KNN, Deep Learning has become a new state-of-the-art method in the field of machine learning.

DL models are systems made up from layers of neurons. Each neuron is a processing unit inspired from existing neurons in the Brain. Every neuron in layer $i$ is connected to all of the neurons in the next layer $i+1$. Output of each neuron is computed as
$ z_{j}^{[i]} = f(w_{j}^{[i]^T}x) + b_{j}{[i]}$, where $z_{j}^{[i]}$ is the output of $j$th neuron of the $i$th layer, $w_{j}^{[i]}$ is the weight matrix, function $f$ is the activation function which introduces a non-linearity \amiraliC{non-linearity or a non-linearity concept (delete "a")} to our model, and $b_{j}^{i}$ is bias. There are various activation functions, such as Sigmoid, 
$$
f(z) = \frac{1}{1 + e^{-z}},
$$
Tanh,
$$
f(z) = \frac{e^z - e^{-z}}{e^z + e^{-z}},
$$
and ReLU,
$$
f(z) = max(0, z)
$$
to mention a few.

The input of the NN is a layer called the input layer. In the training phase, input values are feeded into the model and after computing the loss in the final layer, gradients of the losses are backpropagated to update each layer's weight.

The training data is feeded into the model in small chunks of data called batch. There are many hyperparameters, like number of layers, type of activation function, learning and batch size that have a great impact on the performance of the NN model. These hyperparameters are chosen from a set of predefined set of values and the best values will be selected with respect to the accuracy of the model on validation set.

\subsection{Recurrent Neural Networks}\label{subsec:rnn}
main ref: \cite{hochreiter1997long,chung2014empirical}	
\\
application ref: \cite{vinyals2015show}

The LSTM block is mainly composed of four major components: \begin{inparaenum}
\item Input Gate,
\item Forget Gate,
\item Output Gate, and 
\item the Cell.
\end{inparaenum} These gates, along with element-wise multiplication and summation, allows the LSTM block to calculate its state value, which is stored in the cell component. Furthermore, they generate the output for the LSTM block, which can be fed into another block, or simply to a fully-connected network. The general scheme of an LSTM block at time $t$ is illustrated in the Fig.~\ref{fig:lstmblock}. In the following, each component is briefly introduced and their major functionality is explained.
\subsubsection{The Cell}
{
The state value of the block is stored in the cell, and is updated once a new input is presented to the block. In the Fig.~\ref{fig:lstmblock}, $\mathbf{c^{t-1}}$, showed in the dashed line, refers to the state of the block in time $t-1$, while $\mathbf{c^{t}}$ points to the updated state in time $t$. These state values are used in other gates for properly incorporating the memory and history of prior inputs of the block in the calculations for producing the block's output.
}
 \begin{figure}[!htb] 
 	\centering
%	  \includegraphics[width = 0.9\linewidth]{lstm.pdf}
  \caption{The general block diagram of LSTM.}
  
  \label{fig:lstmblock}
\end{figure}
\subsubsection{Input Gate}
{
At the Input gate, the input values are combined together using a non-linear function, namely Tanh$(.)$, to produce $\mathbf{i^{t}}$, which would be then used for updating the cell state value, $\mathbf{c^{t}}$. Eq.~\ref{eq:input} expresses the function of the input gate formally.
\begin{equation}\label{eq:input}
\mathbf{i^{t}} = \textrm{Tanh}\Big(\mathbf{W_{ix}}\mathbf{x^{t}} + \mathbf{W_{ih}}\mathbf{h^{t-1}} +\mathbf{b}_{i}\Big)
\end{equation}
In Eq.~\ref{eq:input}, $\mathbf{x^{t}}$ refers to the input presented to the block at time $t$, $\mathbf{h^{t-1}}$ is the block's output at time $t-1$, $\mathbf{W_{ih}}$ and $\mathbf{W_{ix}}$ are rectangular weights matrices, and $\mathbf{b}_{i}$ is the bias term.
Furthermore, the \emph{update term}, $\mathbf{z^{t}}$, which determines how the new input values should effect the cell state is calculated. The update term calculations are summarized in Eq.~\ref{eq:update}:
\begin{equation}\label{eq:update}
\mathbf{z^{t}} = \sigma\Big(\mathbf{W_{zx}}\mathbf{x^{t}} + \mathbf{W_{zh}}\mathbf{h^{t-1}} + \mathbf{W_{zc}}\mathbf{c^{t-1}}+\mathbf{b}_{z}\Big)
\end{equation}
where $\sigma(.)$ refers to the \emph{Sigmoid} function, defined as:
\begin{equation}\label{eq:sigmoid}
\sigma(x) = \frac{1}{1+e^{-x}}.
\end{equation}
\amiraliC{We have defined sigmoid before. Maybe delete this definition?} Notice that the block's previous state, $\mathbf{c^{t-1}}$, is also included in the the update term to integrate the history of the cell into calculations.

}
\subsubsection{Forget Gate}
{
In order to update the cell state value, $\mathbf{c^{t}}$, a non-linear function determines how much information from the previous states, encoded in previous cell state value $\mathbf{c^{t-1}}$, should be forgotten, a non-linear function, namely $\sigma(.)$, is deployed. Eq.~\ref{eq:forget} demonstrates the forget gate procedure:
\begin{equation}\label{eq:forget}
\mathbf{f^{t}} = \sigma\Big(\mathbf{W_{fx}}\mathbf{x^{t}} + \mathbf{W_{fh}}\mathbf{h^{t-1}} + \mathbf{W_{fc}}\mathbf{c^{t-1}}+\mathbf{b}_{f}\Big)
\end{equation}
Once the forgot gate value, $\mathbf{f^{t}}$, is calculated, the cell state is updated, integrating the new inputs and also the cell states from previous times using Eq.~\ref{eq:cell}:
\begin{equation}\label{eq:cell}
\mathbf{c^{t}} =
\mathbf{i^{t}}\odot\mathbf{z^{t}} + \mathbf{f^{t}}\odot\mathbf{c^{t-1}}
\end{equation}
In Eq.~\ref{eq:cell}, $\odot$ stands for element-wise multiplication, whereas $+$ refers to vector sum.
}
\subsubsection{Output Gate}
{
At the output gate, the input values combined with the newly updated cell state, are used for calculating the output gate value ($\mathbf{o^{t}}$) as in Eq.~\ref{eq:output}:
\begin{equation}\label{eq:output}
\mathbf{o^{t}} = \sigma\Big(\mathbf{W_{ox}}\mathbf{x^{t}} + \mathbf{W_{oh}}\mathbf{h^{t-1}} + \mathbf{W_{oc}}\mathbf{c^{t}}+\mathbf{b}_{o}\Big)
\end{equation}
Afterwards, the output gate value is again combined with the cell state, which is normalized using a non-linear function, mainly Tanh$(.)$, to produce the cell output value. Eq.~\ref{eq:cell_output} demonstrates this procedure formally:
\begin{equation}\label{eq:cell_output}
\mathbf{h^{t}} =
\mathbf{o^{t}}\odot \textrm{Tanh}\Big(\mathbf{c^{t}}\Big)
\end{equation}

}
There are many LSTM block configurations and setups, each correspond to a particular task. Notice that what was explained here is a more common, basic variation of an LSTM block. As the structure suggests, an LSTM block typically has more parameters, which in return allows [for a more abstract pattern and feature learning]/[them to learn more abstract patterns and features]. However, when using more flexible models, over-fitting phenomenon is more likely to happen. Hence for particular cautions, simplicity of the model must be taken into account.





\subsection{Convolutional Neural Networks}
The convolutional neural networks (CNN) \cite{lecun1995convolutional} are a kind of neural networks that have been successfully applied in areas like image recognition \cite{simonyan2014very} and natural language processing \cite{conneau2016very}. The idea of CNNs is not new; it was originally proposed in ’90s; but due to lack of computational power to train and apply them in real world problems, they were not considered practical until 2011 when the deep learning trend begun.
The convolutional neural networks (CNN) are another type of deep learning models in which feature extraction from the input data is done using layers comprised of convolutional operations. The construction of convolutional networks is inspired by the visual structure of living organisms \cite{hubel1968receptive}. 
%Similar to other kinds of deep learning models, feature extraction plays an essential role in convolutional networks. Features extracted in shallower layers of the convolutional network will be fed to the successive convolutional layers to extract more abstract features. 
Basic building block underneath a CNN is a convolutional layer described as follows:
Consider a convolutional layer with $ N \times N$ square neuron layer as input and a filter $\omega$ of size $m\times m$. The output of this layer $z^l$, is of size $(N-m+1) \times (N-m+1)$ and is computed as follows
\begin{equation}\label{eq:conv_exp}
z_{ij}^\ell =f\left( \sum_{a=0}^{m-1} \sum_{b=0}^{m-1} \omega_{ab} z_{(i+a)(j+b)}^{\ell - 1} \right).
\end{equation}
%This operation is implemented on various deep learning  library ( for example in tensorflow one can use:\\\hspace{-8mm}\numblock{conv2d(x,w,strides,padding).} 
As it is demonstrated in \eqref{eq:conv_exp},
%After the convolution operation, 
usually a non-linear function $f$ such as rectified linear unit (ReLU) is applied to the convolution output to learn more complex features from the data. In some applications, a pooling layer is also applied. The main motivation of employing a pooling layer is to aggregate multiple low-level features in a neighborhood to obtain local invariance. Moreover, it helps to reduce the computation cost of the network in train and test phase.
% train t makes the computations less intensive by down-sampling the data. 
%by the use of making summaries of each sub-region in the output of convolution layers, 
%For example, when using max-pooling, it simply takes some $k \times k$ region and outputs a single value, which is the maximum value of that region. In this case, if the input layer is of size $N \times N$, the pooling layer produces an output of size $\frac{N}{k}\times \frac{N}{k}$, since each $k \times k$ block is reduced to just a single value via the max function.

CNNs have been successfully applied to different fields, including natural language processing \cite{dos2014deep}, computational biology \cite{alipanahi2015predicting}, and machine vision \cite{simonyan2014very}. One of the most interesting applications of CNNs is in face recognition \cite{Lee:2009:CDB:1553374.1553453}, where consecutive convolutional layers are used to extract features from each image. It is observed that the extracted features in shallow layers are simple concepts like edges and curves. On the contrary, features in deeper layers of networks are more abstract than the ones in shallower layers \cite{DBLP:journals/corr/YosinskiCNFL15}. 
However, it is worth mentioning that visualizing the extracted features in the middle layers of a network does not always lead to meaningful concepts like what has been observed in the face recognition task. For example in one-dimensional CNN (1D-CNN) which we use to classify network traffic, the feature vectors extracted in shallow layers are just some real numbers which make no sense at all for a human observer. 

We believe 1D-CNNs are an ideal choice for the network traffic classification task. This is true since 1D-CNNs can capture spatial dependencies between adjacent bytes in network packets that leads to find discriminative patterns for every class of protocols/applications, and consequently, an accurate classification of the traffic. Our classification results confirm this claim and prove that CNNs performs very well in feature extraction of network traffic data.

%====================================================================


==> 05-experiment.tex <==

We want to classify each session just by capturing early packets, so we do not have to wait for the whole session to arrive. Therefore, two different scenarios are designed: in the first scenario, the first 10 raw packets and in the second scenario, the first 10 encrypted packets (i.e. application data) are captured. For the scrappy dataset, we assign the label of traces to be the domain name, and for the selenium dataset, we propose two different labeling schemas, one regarding domain name and another regarding server name. Results of classification accuracies as well as f-scores are presented in the tables \ref{tab:scrappy}, \ref{tab:selenium-domain}, and \ref{tab:selenium-server}.

We have designed 3 different scenarios for fingerprinting. First, all encrypted packets of each session are examined.As mentioned, we do not want to wait for the whole session to conclude. Therefore, the second and third scenario include first 10 packets and second 10 packets of each session, respectively. Results of classification accuracies for each scenario are represented in table \ref{tab:accs} \amiraliC{table???}.

\begin{table}[h]
	\caption{Performance of each model on scrappy dataset}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		& Raw packets & Encrypted packets\\ \hline
		Conv1d &                 &                                                     \\ \hline
		LSTM   &         98.18        &                72.81                                       \\ \hline
		Decision Tree    &         98.58(60)        &          72.01(20)                   \\ \hline
	\end{tabular}
	\label{tab:scrappy}
\end{table}

\begin{table}[h]
	\caption{Performance of each model on selenium dataset (domain name)}
	\begin{tabular}{|c|c|c|c|c|}
	\hline
	& Raw packets & Encrypted packets\\ \hline
	Conv1d &                 &                                                     \\ \hline
	LSTM   &      59.30           &                            43.51                           \\ \hline
	Decision Tree    &        63.25         &         46.62                     \\ \hline
\end{tabular}
	\label{tab:selenium-domain}
\end{table}

\begin{table}[h]
	\caption{Performance of each model on selenium dataset (server name)}
	\begin{tabular}{|c|c|c|c|c|}
	\hline
	& Raw packets & Encrypted packets\\ \hline
	Conv1d &                 &                                                     \\ \hline
	LSTM   &                 &                                                       \\ \hline
	Decision Tree    &                 &                              \\ \hline
\end{tabular}
	\label{tab:selenium-server}
\end{table}

In addition, we propose a new similarity measure between domains within a scope of a finite set of servernames. For each domain $i$, a vector $D_i = <s_{i1}, s_{i2}, ..., s_{im}$ can be defined, where $s_{ij}$ indicates the number of sessions established by domain $D_i$ to servername $s_j$. Given $D_i$ and $D_j$, similarity of these two domains can be defined as the cosine similarity of them,

$$
Sim(D_i, D_j) = \frac{D_i . D_j}{||D_i|| . ||D_j||}, 
$$
where $||.||$ is euclidean distance. Because each element of $D_i$ is greater than or equal to zero, this gives a scalar number which lies between 0 and 1. The more closer this number is to 1, the more request pattern of those domains are similar. In this regard, the maximum similarity between domains was for \textit{addthis.com} and \textit{youtube.com} (0.826), and between \textit{taobao.com} and \textit{tmall.com} (0.822). A clustered heatmap of similarities between each pair of domains is illustrated in figure \ref{fig:sim-all}.

\begin{figure*}[]
	\centering
	\includegraphics[width=0.9\textwidth]{simillarity-of-all.png}
	\caption{Clustered heatmap of similarities between each pair domains}
	\label{fig:sim-all}
\end{figure*}

%\begin{table}[h]
%	\centering
%	\caption{Accuracy of different scenarios}
%	\begin{tabular}{|c|c|c|c|}
%		\hline
%		        & App. data & First 10 packets & Second 10 packets \\ 
%		\hline
%		Scrappy & 76.87\% & 98.77\%         &    \\ 
%		\hline
%		Selenium &                  &                  &                   \\ \hline
%	\end{tabular}
%	\label{tab:accs}
%\end{table}


==> 07-discussion.tex <==
As visible in the experimental results (section~\ref{sec:results}), the data was 


\textit{cutting off headers from the selenium dataset} As the adversary starts sniffing the target's traffic flow, it is possible that he cannot access the initial information of many connections, as the target has established a connection beforehand. For our approach to be applicable in such scenarios, we discard initial packets of every connection (e.g. clienthello, serverhello, ...) when feeding the data to our models and focus only on the application data, making the classification independent of initial packets.

\textit{Why Selenium?} As discussed in section \ref{subsec:sess-des} and \ref{subsec:usr-bhvr}, the only part of a traffic flow that is collected with Scrapy is the initial session. This makes the dataset uniform, as the initial sessions are common and are not convenient for establishing a diversity for classification. The results of \amiraliC{our?} ML \amiraliC{and LSTM?} models show that there needs to be more distinguishing features between different classes to reach a higher accuracy in classification. To address this problem, we also employ Selenium in order to collect all the information stored in Document Object Model (DOM).


==> dataset.tex <==

%\subsubsection{Challenges of data generation}\label{subsubsec:challengesofdatageneration}

The results of this project strongly depend on how well the dataset has been acquired, and the acquisition of comes with various challenges of its own.
Generally speaking, this step consists of two main phases. Traffic generation and Traffic capturing:

\paragraph{Traffic generation}
In this phase, our main goal is to find a way to automatically generate User-like traffic. Our suggested technologies for automated traffic generation are Scrapy and Selenium. In the following we provided advantages for the chosen method.
\paragraph{Traffic capturing}
After generating traffic, the only thing we need is to completely capture and label traffic in several methods. In the other hand, we need a way to fully isolate any Scrapy and Selenium processes traffic for labeling every packets properly. The best solution for this idea is to use operating system network name-spacing technology. For every process that are running in the same time, we assigned unique virtual interface. In this way, we can label every transferred packets through a virtual interface with its corresponding label.

Below is provided a brief explanation for some of these challenges for each phase and how we have act.
\subsubsection{User-like Data Generation (or Data Generation Similar to User's Behaviour)}\label{subsubsec:userlikedatageneration}


Since our system has to work in a realistic situation, our model should be able to classify real users' traffic. So, final tests with this model should be with real users' traffic, and not the artificial traffic generated by crawler.
As previously mentioned, our final experiments were conducted on real traffic. The classification results reproduced with Scrapy dataset surpass that of random choices. But in experimental results we have achieved \ahC{Best accuracy achieved with Scrapy dataset against Scrapy traffic (not real user traffic)} accuracy. It is telling us encrypted traffic generated by Scrapy  is much enough learnable and can be easily classify.  We conclude that the traffic generated using Scrapy differed compared to real users' traffic. So we decided to change the way we generate traffic. In a real situation, as the user starts to surf the web with a browser, the browser is supposed to send all requests that are mentioned in the requested webpage HTML source. Also, the browser should run all Javascript codes related to the page with its engine, which can lead to sending more requests. Hence, if we send only the first request to receive the original HTML source, other parts of a page will not be downloaded and the traffic will be limited in a non-realistic manner -- which is what Scrapy does. This way we leave important parts of traffic out of what is collected, such as pictures, videos, Javascript requests, and other components that are stored in HTML DOM (Document Object Model). On another note, in some situations the browser makes the decision to redirect a page to another, and these situations get neglected during this method. So we needed another approach to gather all components of a page like a browser. In fact we need a way to completely give browsers control. One way to achieve this is to use browsers' driver, which led us to the inclusion of Selenium.

Selenium is a tool that can communicate with different browsers' driver and gives the user full control over the browser. After redesigning the crawler with the inclusion of selenium and collecting traffic afterwards, we trained our model again. This time, the experimental results was worse than the previous method.As previously mentioned, in real situation, user will try to send several requests correspond to different servers (such as advertisement services requests) even if surfing a single page, which leads to collecting miscellaneous traffic along with the traffic we intended to collect. So we can understand this is on of the reasons for reduction of accuracy. Different patterns from unknown websites will factor into our neural network's training phase. This way, every website's fingerprint will be composed of patterns from and not from that website, which leads to our classifier not being able to distinguish between different classes as well. But in final experiments, as expected, our new model can better classify users behaviours. Because in this way we completely simulate users actions while surfing the web.

So, the next idea was to up the accuracy by making the collected traffic pure. As referred above, any single page traffic consist of a dynamic set of different sessions. Hence, we decide to label every session with its own server name, and we tried to train our model with new labeling method. In Transport Layer Security, there is several kind of packets for starting new TLS session. At first, client tries to establish new connection with sending server a new Client Hello packet. In this packet there is a field named Server Name that will tell the server host which service we are looking for. With this new labeling method, we can rise up our accuracy well. Also, the traffic in final experiment was well enough like to real user traffic.
\\
We used chrome browser's driver via Selenium for generating traffic. The process ran on two systems with 12 separate threads, Every thread crawled a domain with 100 random pages separately in a unique namespace every time and collected the traffic. On average, there are about 2000 pages crawled from every domain in 100 page batches. Also there is a 6 second delay between collecting every page, so the destination server does not recognize the crawler as a bot. The traffic generation process takes about 3 month long.

Even without considering user's behaviour and analyzing only the traffic collected by the crawler, another problem is traffic expiration, meaning the traffic's cryptography will change after a period. We have found a way to resolve this problem \amiraliC{to-do: add Solution explanation (Amirmohammad)}.

As mentioned, time related meta-data should not be factored in the classifier. Main reason is that these features are dependent not only on the destination website, but they also rely on information exchange platform, internet speed, etc., none of which are related to the destination website and can reduce our accuracy. Even if we use the packets' length as a meta-data (?), unrelated factors - like information exchange platform - could influence our classification, as the way data is fragmented and forwarded to user is based on information exchange platform; as the result, final pattern will be influenced by these alterations in the database.





%
%
%The results of this project strongly depend on how well the dataset has been acquired, and the acquisition of comes with various challenges of its own.
%Generally speaking, this step consists of two main phases. Traffic generation and Traffic capturing:
%
%In this phase, our main goal is to find a way to automatically generate User-like traffic. Our suggested technologies for automated traffic generation are Scrapy and Selenium. In the following, we provided advantages for the chosen method.
%\paragraph{Traffic capturing}
%After generating traffic, the only thing we need is to completely capture and label traffic in several methods. In the other hand, we need a way to fully isolate any Scrapy and Selenium processes traffic for labeling every packet properly. The best solution for this idea is to use operating system network name-spacing technology. For every process that is running at the same time, we assigned a unique virtual interface. In this way, we can label every transferred packet through a virtual interface with its corresponding label.
%
%What follows is a brief explanation for some of these challenges concerning each phase and its suggested solutions.
%\subsubsection{User-like Data Generation (or Data Generation Similar to User's Behaviour)}\label{subsubsec:userlikedatageneration}
%
%
%Since our system has to work in a realistic situation, our model should be able to recognize real users' behavior. So, final tests of this model should be done with real users' traffic, and not the artificial traffic generated by the crawler.
%As previously mentioned, our final experiments were conducted on real traffic. The classification results produced with Scrapy dataset surpass that of random choices. But in experimental results we have achieved \ahC{Best accuracy achieved with Scrapy dataset against Scrapy traffic (not real user traffic)} accuracy. It is telling us encrypted traffic generated by Scrapy  is much enough learnable and can be easily classify.  We conclude that the traffic generated using Scrapy differed compared to real users' traffic. So we decided to change the way we generate traffic. In a real situation, as the user starts to surf the web with a browser, the browser is supposed to send all requests that are mentioned in the requested webpage HTML source. Also, the browser should run all Javascript codes related to the page with its engine, which can lead to sending more requests. Hence, if we send only the first request to receive the original HTML source, other parts of a page will not be downloaded and the traffic will be limited in a non-realistic manner -- which is what Scrapy does. This way we leave important parts of traffic out of what is collected, such as pictures, videos, Javascript requests, and other components that are stored in HTML DOM (Document Object Model). On another note, in some situations, the browser makes the decision to redirect a page to another, and these situations get neglected during this method. So we needed another approach to gather all components of a page like a browser. In fact, we need a way to completely give browsers control. One way to achieve this is to use browsers' driver, which led us to the inclusion of Selenium.
%
%Selenium is a tool that can communicate with different browsers' driver and gives the user full control over the browser. After redesigning the crawler with the inclusion of selenium and collecting traffic afterwards, we trained our model again. This time, the experimental results was worse than the previous method.As previously mentioned, in real situation, user will try to send several requests correspond to different servers (such as advertisement services requests) even if surfing a single page, which leads to collecting miscellaneous traffic along with the traffic we intended to collect. So we can understand this is on of the reasons for reduction of accuracy. Different patterns from unknown websites will factor into our neural network's training phase. This way, every website's fingerprint will be composed of patterns from and not from that website, which leads to our classifier not being able to distinguish between different classes as well. But in final experiments, as expected, our new model can better classify users behaviours. Because in this way we completely simulate users actions while surfing the web.
%
%So, the next idea was to up the accuracy by making the collected traffic pure. As referred above, any single page traffic consist of a dynamic set of different sessions. Hence, we decide to label every session with its own server name, and we tried to train our model with new labeling method. In Transport Layer Security, there is several kind of packets for starting new TLS session. At first, client tries to establish new connection with sending server a new Client Hello packet. In this packet, there is a field named Server Name that will tell the server host which service we are looking for. With this new labeling method, we can rise up our accuracy well. Also, the traffic in final experiment was well enough like to real user traffic.
%\\
%We used chrome browser's driver via Selenium for generating traffic. The process ran on two systems with 12 separate threads, Every thread crawled a domain with 100 random pages separately in a unique namespace every time and collected the traffic. On average, there are about 2000 pages crawled from every domain in 100-page batches. Also, there is a 6-second delay between collecting every page, so the destination server does not recognize the crawler as a bot. The traffic generation process takes about 3 months long.
%
%Even without considering the user's behavior and analyzing only the traffic collected by the crawler, another problem is traffic expiration, meaning the traffic's cryptography will change after a period. We have found a way to resolve this problem \amiraliC{to-do: add Solution explanation (Amirmohammad)}.
%
%As mentioned, time-related meta-data should not be factored in the classifier. The main reason is that these features are dependent not only on the destination website, but they also rely on the information exchange platform, internet speed, etc., none of which are related to the destination website and can reduce accuracy. Even if we use the packets' length as a meta-data (?), unrelated factors - like information exchange platform - could influence our classification, as the way data is fragmented and forwarded to user is based on information exchange platform; as the result, the final pattern will be influenced by these alterations in the database.

